RISCORE: Enhancing In-Context Riddle Solving in Language Models through Context-Reconstructed Example Augmentation

Riddle-solving requires advanced reasoning skills, pushing LLMs to engage in abstract thinking and creative problem-solving, often revealing limitations in their cognitive abilities. In this paper, we examine the riddle-solving capabilities of LLMs using a multiple-choice format, exploring how different prompting techniques impact performance on riddles that demand diverse reasoning skills. To enhance results, we introduce RISCORE (RIddle Solving with COntext REcontruciton) a novel fully automated prompting method that generates and utilizes contextually reconstructed sentence-based puzzles in conjunction with the original examples to create few-shot exemplars. Our experiments demonstrate that RISCORE significantly improves the performance of language models in both vertical and lateral thinking tasks, surpassing traditional exemplar selection strategies across a variety of few-shot settings.

==> images/figs/fig1.tex <==
\begin{figure*}[ht!]
\centering
    \includegraphics[width=0.8\textwidth]{images/prompting_tree.png}
\vskip -0.01in
\caption{We demonstrate an example of few-shot (FS) prompting alongside the same method using a context-reconstructed example. The text in green represents the context reconstruction of Example 1, produced by the proposed method. The example in red was removed simply to maintain the same number of shots.}
\label{fig:method}
\end{figure*}


\begin{figure*}[ht!]
\centering
\includesvg[width=0.8\textwidth]{images/riscore_pipeliine.drawio.svg}
\vskip -0.01in
% \caption{An example of RISCORE utilizing 2-shot prompting. The test riddle (\textbf{TR}) is compared in \textbf{vector space} to other riddles, with \textbf{R1} and \textbf{R2} being the most semantically similar. RISCORE reconstructs \textbf{R1} (\textbf{R1CR}) and \textbf{R2} (\textbf{R2CR}), introducing the same reasoning in a new context. The contextually reconstructed riddles and the original ones are used in a \textbf{few-shot prompt} for \textbf{LM inference}.}
\label{fig:example}
\end{figure*}


\begin{figure}[ht!]
\centering
\includesvg[width=\columnwidth]{images/riscore.drawio.svg}
\vskip -0.01in
\caption{An example of RISCORE utilizing 2-shot prompting. The test riddle (\textbf{TR}) is compared in \textbf{vector space} to other riddles, with \textbf{R1} and \textbf{R2} being the most semantically similar. RISCORE reconstructs \textbf{R1} (\textbf{R1CR}) and \textbf{R2} (\textbf{R2CR}), introducing the same reasoning in a new context. The contextually reconstructed riddles and the original ones are used in a \textbf{few-shot prompt} for \textbf{LM inference}.}
\label{fig:example}
\end{figure}

